An unbiased ray-marching transmittance estimator

We present an in-depth analysis of the sources of variance in state-of-the-art unbiased volumetric transmittance estimators, and propose several new methods for improving their efficiency. These combine to produce a single estimator that is universally optimal relative to prior work, with up to several orders of magnitude lower variance at the same cost, and has zero variance for any ray with non-varying extinction. We first reduce the variance of truncated power-series estimators using a novel efficient application of U-statistics. We then greatly reduce the average expansion order of the power series and redistribute density evaluations to filter the optical depth estimates with an equidistant sampling comb. Combined with the use of an online control variate built from a sampled mean density estimate, the resulting estimator effectively performs ray marching most of the time while using rarely-sampled higher order terms to correct the bias.

==> contribs.tex <==


%------------------------------------------------------------
\section{Contributions}
%------------------------------------------------------------

% Breakdown: I'm guessing we will evaluate two major themes, which we could call \emph{blind} and \emph{informed}.  Blind transmittance estimation is when we don't exploit any data structure over the densities and know nothing more than min, max, mean and possibly variance of the densities in the entire volume.  A lot of what we have done so far seems to relate to the optimal estimator for blind transmittance estimation and closely relates to prior variance and efficiency studies.

% We can also consider informed estimation, where we have more information about the density along a given path before we start taking any samples.  Piecewise-linear or cubic approximations, etc, which Jan has set up is one version of this.

\paragraph{Reminder list of contributions}

    \begin{compactitem}
        \item derivation of zero-variance ratio tracking
        \item derivation of zero-variance next-flight ratio tracking
        \item exact expression for variance and efficiency for residual ratio tracking - from this we find the minimum-variance constant control for residual ratio tracking (for constant control and majorant) - and also note that RT is optimally efficient with infinite majorant 
        \item observation: control term in residual tracking yields exponential transform - I think another paper hints at this, actually (eug: TODO)
        \item highlight important related work between nonhomogeneous Poisson point process sampling and delta tracking (thinning)
        \item highlight important related work of Bhanot Kennedy, Wagner
        \item highlight relevant prior art intentionally uncited by \cite{georgiev2019integral}: \cite{elhafi2018three}
        \item introduce rotation and permutation power-series estimators and explore their properties 
        \item introduce efficient (Girard-Newtown) and numerically stable methods for computing fully-permuted power-series estimators
        \item discuss link with \cite{lee2019unbiased} using polynomial factorization?
        \item we provide a more comprehensive efficiency analysis of the various transmittance estimators than prior work 
        \item comb tuples with affine end-point alignment
        \item discuss sample-tuple-based estimation with intra-tuple stratification, and why global stratification would bias the power series estimator (reference \cite{raab2006unbiased})
        \item (Markus) I propose not talking about density samples and tuples, but independent unbiased estimates for the density integral
        \item (Markus) Dress affine CV and equidistant sampling as \emph{density reshuffling} to help the analysis and help implementing new methods
        \item higher order stratification (across multiple evaluations)
        \item ratio tracking where the constant term is transformed to an expected value
        \item jackknife for biased estimators
        \item relationship to work in statistics - Johnson et al.
    \end{compactitem}
    
    % Opens questions:
    % \begin{compactitem}
    %     \item (eug) I saw numerical issues with one of my Girard Newton variants that remaps values to avoid overflowing the float range
    %     \subitem (Markus) Solution: Numerical issues are resolved by normalizing the samples such that the highest absolute value is 1 before evaluating the symmetric sums (this needs to be undone at the time of evaluation of the Taylor series; $c := c / (1+i)$ becomes $c := c * L / (1 + i)$ where $L$ is the normalization factor. In addition, we have code to directly evaluate elementary symmetric means. However, after the most aggressive roulettes these should no longer be a problems due to the low orders of evaluation, but the basic combination estimator without density reshuffling certainly benefits from these improvements. 
    % \end{compactitem}
